LLMs-as-Instructors: Learning from Errors Toward Automating Model Improvement

This paper introduces the innovative "LLMs-as-Instructors" framework, which leverages the advanced Large Language Models (LLMs) to autonomously enhance the training of smaller target models. Inspired by the theory of "Learning from Errors", this framework employs an instructor LLM to meticulously analyze the specific errors within a target model, facilitating targeted and efficient training cycles. Within this framework, we implement two strategies: "Learning from Error," which focuses solely on incorrect responses to tailor training data, and "Learning from Error by Contrast", which uses contrastive learning to analyze both correct and incorrect responses for a deeper understanding of errors. Our empirical studies, conducted with several open-source models, demonstrate significant improvements across multiple benchmarks, including mathematical reasoning, coding abilities, and factual knowledge. Notably, the refined Llama-3-8b-Instruction has outperformed ChatGPT, illustrating the effectiveness of our approach. By leveraging the strengths of both strategies, we have attained a more balanced performance improvement on both in-domain and out-of-domain benchmarks. Our code can be found at https://yingjiahao14.github.io/LLMs-as-Instructors-pages/.

==> chapters/instro_1_pre.tex <==
\section{Introduction}
\iffalse
The training of Large Language Models (LLMs) is a human-in-the-loop process. In this process, developers continuously analyze the model's responses and use these insights to modify the training corpus or supplement the dataset. This rigorous training regimen is notably time-consuming and labor-intensive.
Recent advancements have unveiled that certain advanced LLMs, such as GPT-4~\cite{GPT-4} and Claude-3~\cite{claude-3}, which have been nurtured on expansive corpora, exhibit exceptional analytical, evaluative, and data generation competencies~\cite{bai2023benchmarking,dai2023auggpt,xu2023wizardlm}. It is therefore pertinent to explore the possibility of using LLMs to autonomously analyze the target model's response, adjust the training corpus, and supplement the dataset in the training phase, thereby enhancing the LLMs' performance with minimal human intervention.
\fi

Training Large Language Models (LLMs) is notably time-consuming and labor-intensive. In this process, developers continuously analyze the model's responses and use these insights to modify the training corpus or supplement the dataset. 


\begin{figure}[t]
\centering
\includegraphics[scale=0.36]{figure/intro_2.pdf}
%    \vspace{-1mm}
    \caption{Compared with previous traditional data augmentation method~\cite{dai2023auggpt, xu2023wizardlm} --- used stronger models to generate training data without considering the target model's features, we propose an LLMs-as-Instructor framework based on the ``Learning from Errors'' theory~\cite{metcalfe2017learning}, where a stronger model analyzes and targets the specific errors of a smaller model to facilitate direct improvements.}
    \label{fig: intro}  
%\vspace{-4mm}
\end{figure}

However, current attempts are predominantly confined to simplistic applications --- employing advanced LLMs for tasks such as data augmentation~\cite{dai2023auggpt}, training corpus generation~\cite{xu2023wizardlm}, and data annotation~\cite{rafailov2024direct} --- which fail to leverage LLMs' full analytical capabilities and potential for automation. On the other hand, these general applications do not target specific features of the model for enhancement, which, according to~\citet{bloom19842}, could be an efficient way to enhance LLMs learning, as it is for humans. Figure\,\ref{fig: intro} illustrates an example where the target model encounters issues in maintaining computational precision. Indiscriminately adding additional instructions could lead to inefficient improvements.  Conversely, utilizing the model’s specific errors in maintaining precision for targeted enhancement could be more focused and consequently more effective.




 
Therefore, in this work, we tailor the advanced LLMs to serve as instructors that analyze the target model based on its features and supplement training materials to facilitate improvements. Inspired by the theory of ``Learning from Errors'' as discussed in~\citet{metcalfe2017learning}, which posits that learning from errors deepens understanding and memory, we focus the instructor model on the errors of the target model to enhance its learning process effectively.

% To this end, we establish an ``LLMs-as-Instructors'' framework, where the instructor LLM takes the responses of the target models as input then analyzes the responses to identify areas of improvement and supplements corresponding training materials to refine the model. We select three open-source LLMs as the target model can conduct experiment, we achieve.
% The instructor then uses supplemental data samples to iteratively train the target models.
% We aim to answer the following questions:
Taking into account the above insights, we establish an ``LLMs-as-Instructors'' framework, where the instructor LLM takes the responses of the target models as input to assess the state of the target model and then generates training materials to help improve the model. To better guide the target model, we set two analysis strategies: \textbf{1) Learning from Error:} where the instructor only analyzes the erroneous responses,
and \textbf{2) Learning from Error by Contrast:} considering the concept of contrastive learning in machine learning, we refine the identification of the model's deficiencies by adding some correct samples on top of the ``Learning from Error'' approach. This allows the instructor to help comprehensively analyze.
%
Our experiments, utilizing the open-source Mistral-7b-Instruct model\cite{mistral-7b}, have demonstrated that after three iterative training cycles, our LLMs-as-Instructors framework significantly enhances the baseline target model across various benchmarks, regardless the strategy employed. The outcomes reveal that each strategy offers unique benefits contigent upon the nature of the data. In contexts where the question samples are granular and there is an abundance of both correct and incorrect cases, the use of contrast samples substantially benefits the Instructor. On the other hand, for more general and less frequent questions, the ``Learning from error'' strategy is directly more efficacious in augmenting the model's capabilities. By combining the strengths of both strategies, we have realized a more balanced improvement in performance on both in-domain and out-of-domain benchmarks.
%


Our main contributions can be summarized as:
\setlist[itemize]{left=0pt}
\begin{itemize}
%   \vspace{-2mm} 
    \item We have proposed the LLMs-as-Instructors framework, which leverages the capabilities of advanced LLMs to autonomously analyze the characteristics of the target model and enhance it through iterative training cycles.
%    \vspace{-2mm}
    \item We have introduced and effectively implemented two distinct analysis strategies: ``Learning from Errors'' and ``Learning from Errors by Contrast,'' which are adaptable to various scenarios and facilitate learning from errors.
%    \vspace{-2mm}
    \item  Our evaluation spans multiple benchmarks and diverse domains, including factual knowledge, mathematical reasoning, and coding, confirming that our framework significantly improves the performance of target models.
%    \vspace{-2mm}
\end{itemize}




==> chapters/instroduction.tex <==
\section{Instruction}
Large Language Models (LLMs) have become essential tools in the field of Natural Language Processing (NLP), marking significant advancements as highlighted by a series of influential studies~\citep{brown2020language, weichain, mirowski2023co}. Trained on wide-ranging datasets, these models exhibit remarkable emergent abilities, including in-context learning, instruction following, and step-by-step reasoning capabilities~\citep{wei2022emergent, zhao2023survey}. As the capabilities of LLMs expand, a diverse array of benchmarks has been developed to comprehensively assess these models' abilities~\citep{srivastava2023beyond, hendryckstest2021,zhong2023agieval, cobbe2021training}. 

However, along with this explosion of open-source benchmarks, a critical issue, data leakage or contamination, has been raised ~\citep{li2023open, zhou2023don, wei2023skywork, li2023task, jacovi2023stop}.  Data contamination refers to the phenomenon that examples from the evaluation set are also found in the training set~\citep{li2023open}. This issue can happen when the evaluation datasets are constructed on the training corpus of the LLMs. Highlighted in recent studies~\citep{zhou2023don}, under the effect of the data contamination, the integrity and reliability of the evaluation result are compromised. 
\begin{figure}[t]
\centering
\includegraphics[scale=0.68]{figures/intro_1.pdf}
    \caption{Auto-question generation framework. }
    \label{fig: intro}  
\vspace{-5mm}
\end{figure} 
Strategies to alleviate the data leakage problem, such as: avoiding data that appears with its solution on the internet or encrypting the test sample to prohibit distribution of adaptations~\citep{jacovi2023stop} are costly and cumbersome in their implementation.

In response to these challenges, this study introduces an auto-question answer generation framework. This framework is designed to dynamically generate new, uncontaminated evaluation question samples, offering a cost-effective and efficient solution to mitigate the issue of dataset leakage. Our framework proceeds in two settings: \textbf{1. Mimic }, where we leverage LLMs to replicate data samples from existing benchmarks. The aim is to generate new samples efficiently while preserving the stylistic and contextual essence of the original data. \textbf{2. Extend }, where we enhance the existing samples with varying cognitive levels, thereby creating new and more intricately fine-grained samples. 

With testing on 6 open-source models and 4 closed-source models, we find that:
% 1. The Mimic method is stable and shows robustness against the data leakage problem, though affected by the problem learning the answer distribution 2. By deploying extend setting we can get new questions that nearly have no datt contamination problem 3. Using different cognifition -level and difere popoluritiy as the seed we can control the difficult of the question thus
\textbf{1. Stability of the Mimic Setting:} Mimic setting demonstrates a high level of stability in maintaining the quality of generated questions and exhibits robustness against data leakage issues. However, it is susceptible to the challenge of models’ learning of the answer distribution. 
\textbf{2. Effectiveness of the Extend Setting:} The extend setting proves to be highly effective in generating new questions with minimal data contamination. This approach significantly mitigates the risk of data leakage, enhancing the reliability of the evaluation process. 
\textbf{3. Difficulty Controllable Question Generation:} By varying the cognitive level and the popularity of the seed used for question extention, we can effectively modulate the difficulty of the questions. 






==> chapters/intro.tex <==
\section{Introduction}
\iffalse
The training of Large Language Models (LLMs) often involves a human-in-the-loop process. LLMs, which consist of a significantly larger number of parameters, require extensive training data that covers a broad range of content during the pre-training stage. For this purpose, developers may collect trillions of tokens from accessible training datasets. After pre-training, it is necessary to fine-tune LLMs to enhance their capacity. This stage often involves developers designing and collecting question-answer pairs to improve the model's understanding of instructions and better align it with human preferences. Besides the data collecting and processing, developers may use feedback from the model to adjust the training corpus and supplement training samples. This entire training process is extensive and costly.


On the other hand, recent work has shown that sophisticated LLMs like GPT-4~\cite{GPT-4} and Claude-3~\cite{claude-3}, which have been trained on extensive corpora, demonstrate remarkable analytical and evaluative abilities as well as data generation capabilities.
Naturally, this leads us to consider whether it is possible to replace human roles in training with models that can analyze, collect, and supplement data, thus autonomously improving the LLMs.
\fi



The training of Large Language Models (LLMs) typically incorporates a human-in-the-loop process, wherein human involvement is pivotal in both the training phase and the verification of the model's performance. These models, endowed with an immense array of parameters, demand a voluminous training dataset that spans a diverse spectrum of content during the initial pre-training phase. To this end, developers might curate an extensive corpus by harvesting trillions of tokens from publicly accessible datasets~\cite{Gokaslan2019OpenWeb, pile}.  
%
Post the pre-training phase, the imperative task of fine-tuning LLMs, arises to amplify their capabilities~\cite{longpre2023flan, wang2024far}. This phase frequently entails the formulation and aggregation of question-answer pairs by developers, which serves to enhance the model's comprehension of directives and to harmonize it more closely with human inclinations. 
%
%
% In addition to data aggregation and refinement, developers may also harness feedback from the model to calibrate the training corpus and enrich the training data. 

\iffalse
During these two training phases, developers also harness feedback from the model's performance/response to dynamically adjust the training corpus and supplement the training data, thereby further refining the model’s capabilities.
This comprehensive training regiment is notably elaborate and financially demanding.
\fi

Throughout the two training phases, developers must meticulously monitor the model's feedback and performance. They should be prepared to modify the training corpus or supplement the dataset to enhance the model's proficiency. This rigorous training regimen is notably intricate and requires substantial financial investment.
%
Conversely, recent advancements have unveiled that certain advanced LLMs, such as GPT-4~\cite{GPT-4} and Claude-3~\cite{claude-3}, which have been nurtured on expansive corpora, exhibit exceptional analytical, evaluative, and data generation competencies. It is therefore pertinent to explore the possibility of automating the training process with models that can autonomously analyze their own characteristics, adjust the training corpus, and supplement the dataset, thereby enhancing the LLMs' performance without human intervention.



%
\iffalse
On the other hand, recent advancements have unveiled that certain advanced LLMs, such as GPT-4~\cite{GPT-4} and Claude-3~\cite{claude-3}, which have been nurtured on expansive corpora, exhibit exceptional analytical, evaluative, and data generation competencies. Consequently, it is natural to consider whether it is possible to replace human roles in training with models that can analyze the model's characteristics, adjust the training corpus, and supplement the training data, thus autonomously improving the LLMs.
%
\fi

However, current attempts are predominantly confined to simplistic applications --- employing these advanced LLMs for tasks such as data augmentation~\cite{dai2023auggpt}, training corpus generation~\cite{xu2023wizardlm}, and data annotation~\cite{rafailov2024direct}. These applications have yet to fully delve into the autonomous exploitation of the LLMs' capacity to adapt to the unique requirements and attributes of the models undergoing training.

%
% Instead, a more strategic approach is needed to harness the full capabilities of these LLMs for generating data that is specifically tailored to the models being trained.
%
%
%
%this naturally prompts the contemplation of whether the human element in training can be supplanted by models that are capable of autonomously analyzing, amassing, and augmenting data, thereby continuously refining the LLMs.




\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{figure/intro.pdf}
%    \vspace{-1mm}
    \caption{Previous work~\cite{dai2023auggpt, xu2023wizardlm} used stronger models to assist in training but did not specifically enhance the target model based on its errors (Non-Discriminative Learning). We propose an ``LLMs-as-Instructor'' framework based on the "Learning from Errors" theory~\cite{metcalfe2017learning}, where a stronger model analyzes and targets the specific errors of a smaller model to facilitate direct improvements.}
    \label{fig: intro}  
   \vspace{-4mm}
\end{figure} 


In this work, we explore the potential of LLMs to serve as instructors during training our language model, with particular efforts to recognizing the capability of our model. Specifically, we focus on the fine-tuning stage and investigate whether superior LLMs can analyze the responses from target models and autonomously improve their performance. 
Inspired by the human effective learning method ``Learning from Errors'' as discussed in the work~\cite{metcalfe2017learning}, which posits that learning from mistakes helps deepen understanding and memory, we set target models to learn from their errors.
To this end, we establish an ``LLMs-as-Instructors'' framework, where the instructor LLM takes the responses of the target models as input then analyzes the responses to identify areas of improvement and supplements corresponding training materials to refine the model. We select three open-source LLMs as the target model can conduct experiment, we achieve.
% The instructor then uses supplemental data samples to iteratively train the target models.
% We aim to answer the following questions:



Our main contributions can be summarized:
\begin{itemize}
   \vspace{-2mm}
    \item 
    \vspace{-2mm}
    \item 
    \vspace{-2mm}
    \item 
    \vspace{-2mm}
\end{itemize}
